Pooling Representation Autoencoders for Efficient Diffusion

Representation Autoencoders (RAEs) generate images from pre-trained visual fea- tures, but their dense token grids make generative modeling expensive. Motivated by local feature correlations, we introduce PoolDINO, a learned affine pooling operator that merges neighboring tokens. Training the pooling operator jointly with the RGB decoder preserves the standard two-stage RAE procedure without a separate feature auto-encoder. On ImageNet-256, 4x token compression retains comparable generation quality under internal guidance, while 16x compression trades some quality for greater efficiency. At a fixed budget of 100 sampling steps, latent-sampling throughput increases by 3.7x and 9.0x, respectively, relative to the unpooled baseline. Classification and dense prediction evaluations show that comparable guided generation quality can coexist with weaker performance on other tasks.

==> figures/quality_throughput_literature_points.tex <==
% External baselines retain their original FIDs, throughput, and timing SDs.
\addplot[only marks,black!50,mark=diamond*,mark size=2.2pt,
    forget plot,error bars/.cd,x dir=both,x explicit] coordinates {
    (6.140202012224861,1.67) +- (0.0022831176485612306,0)
    (12.333923401332111,1.78) +- (0.019504329331953216,0)
    (22.25987542683997,2.44) +- (0.07407767770274822,0)
    (3.1383672813042254,1.42) +- (0.000657529677442022,0)
    (1.2310240113665198,1.55) +- (0.004902102944190099,0)
    (14.820128554110196,1.13) +- (0.017648222970774795,0)
    (2.7346668802603142,1.35) +- (0.0008613857960049152,0)
    (3.0745529762099024,1.12) +- (0.0008952060899096071,0)
};
% Direct labels use opposite sides of the two closest baseline points.
\begin{scope}[every node/.style={font=\scriptsize,
    text=black!60,fill=white,inner sep=1pt}]
\node[anchor=south east,xshift=-3pt,yshift=3pt]
    at (axis cs:6.140202012224861,1.67) {MAETok (128)};
\node[anchor=south east,xshift=-3pt,yshift=5pt]
    at (axis cs:12.333923401332111,1.78) {SoftVQ (64)};
\node[anchor=north east,xshift=-3pt,yshift=-3pt]
    at (axis cs:22.25987542683997,2.44) {SoftVQ (32)};
\node[anchor=west,xshift=5pt]
    at (axis cs:3.1383672813042254,1.42) {REPA};
\node[anchor=east,xshift=-4pt,yshift=1pt]
    at (axis cs:1.2310240113665198,1.55) {MAR-H};
\node[anchor=south east,xshift=-4pt,yshift=4pt]
    at (axis cs:14.820128554110196,1.13) {RAE};
\node[anchor=east,xshift=-4pt]
    at (axis cs:2.7346668802603142,1.35) {LightningDiT};
\node[anchor=east,xshift=-4pt]
    at (axis cs:3.0745529762099024,1.12) {REPA-E};
\end{scope}


==> figures/sampling_steps_data.tex <==
% Fixed IG=2.75, learned 4x4 pooling, 300 training epochs.
% Source: logs/FIFTY_STEP_GENERATION_RESULTS.tex.
\pgfplotstableread{
steps fid is
10 2.4756 224.15
20 1.4862 245.74
30 1.3611 250.39
40 1.3191 252.49
50 1.2981 255.25
100 1.2882 258.04
}\poolSamplingStepsData

